Graph Fourier Transform with Negative Edges for Depth Image Coding

Recent advent in graph signal processing (GSP) has led to the development of new graph-based transforms and wavelets for image / video coding, where the underlying graph describes inter-pixel correlations. In this paper, we develop a new transform called signed graph Fourier transform (SGFT), where the underlying graph G contains negative edges that describe anti-correlations between pixel pairs. Specifically, we first construct a one-state Markov process that models both inter-pixel correlations and anti-correlations. We then derive the corresponding precision matrix, and show that the loopy graph Laplacian matrix Q of a graph G with a negative edge and two self-loops at its end nodes is approximately equivalent. This proves that the eigenvectors of Q - called SGFT - approximates the optimal Karhunen-Lo`eve Transform (KLT). We show the importance of the self-loops in G to ensure Q is positive semi-definite. We prove that the first eigenvector of Q is piecewise constant (PWC), and thus can well approximate a piecewise smooth (PWS) signal like a depth image. Experimental results show that a block-based coding scheme based on SGFT outperforms a previous scheme using graph transforms with only positive edges for several depth images.

==> related.tex <==
\vspace{-0.05in}
To exploit the unique \textit{piecewise smooth } (pws) characteristic in depth images, new transforms and wavelets have been proposed for efficient comprssion \cite{maitre08,shen10pcs}.

\cite{shen10pcs} proposed a new graph-based transform where 

\cite{zhang13}

An extension of \cite{shen10pcs}, \cite{hu15} proposed a new multi-resolution graph transform approach, where one key contribution is the proof of optimality of the GFT for a one-state Markov model.
In particular, to model a signal discontinuity (sharp edge in a depth image) from pixel $x_{k-1}$ to $x_k$, \cite{hu15} assume a non-zero-mean variable $z_k$ with a different variance than other pixel pairs. 

Our work extends from \cite{hu15}

\cite{hu15spl}
